When is an Embedding Model More Promising than Another?

Embedders play a central role in machine learning, projecting any object into numerical representations that can, in turn, be leveraged to perform various downstream tasks. The evaluation of embedding models typically depends on domain-specific empirical approaches utilizing downstream tasks, primarily because of the lack of a standardized framework for comparison. However, acquiring adequately large and representative datasets for conducting these assessments is not always viable and can prove to be prohibitively expensive and time-consuming. In this paper, we present a unified approach to evaluate embedders. First, we establish theoretical foundations for comparing embedding models, drawing upon the concepts of sufficiency and informativeness. We then leverage these concepts to devise a tractable comparison criterion (information sufficiency), leading to a task-agnostic and self-supervised ranking procedure. We demonstrate experimentally that our approach aligns closely with the capability of embedding models to facilitate various downstream tasks in both natural language processing and molecular biology. This effectively offers practitioners a valuable tool for prioritizing model trials.

==> philippe_pres/1_intro.tex <==

\section{What are embeddings Models?}

    \begin{frame}{Different molecular modalities}

        \begin{columns}
            \begin{column}{0.4\linewidth}
                An embedder is a function that maps an object to a vector space.

                This representation can be used to perform various downstream tasks (property prediction, docking, \ldots)
            \end{column}

            \begin{column}{0.6\linewidth}
                \begin{figure}
                    \centering
                    \includegraphics[width=\linewidth]{talk_figs/repres_mol}
                    \caption{Illustration of three different molecular modalities used to embed molecules.}
                    \label{fig:repres_mol}
                \end{figure}
            \end{column}

        \end{columns}
    \end{frame}


    \begin{frame}{Different molecular modalities}

        To process molecular data, various embedding models have been proposed for each data modality.:

        \begin{itemize}
             \item \textbf{Sequence-based models}: Masked modeling objectives, Regressive objectives\cite{ahmad2022chemberta2}, etc.
            \item \textbf{2D-Graph-based models}: AttributeMasking, ContextPred\cite{sun2022does}, MolR\cite{wang2022chemicalreactionaware}, etc.
            \item \textbf{3D-Graph-based models}: Transformer-M\cite{luo2023one}, SE(3)-DDM\cite{liu2023molecular}, FRAD\cite{pmlr-v202-feng23c}, etc.
            \item \textbf{Hybrid models}: GraphMVP\cite{liu2022pretraining}, ThreeDInfomax\cite{stark2021_3dinfomax}, etc.
        \end{itemize}

    \end{frame}

    \begin{frame}{Limitations of embedding evaluation}
        The comparison of embedding models is typically done through downstream tasks, which has two main limitations:
        \begin{itemize}
            \item \textbf{Costly}: Acquiring adequately large and representative datasets can be prohibitively expensive and time-consuming.
            \item \textbf{Un-interpretable}: The evaluation of embedding models typically depends on domain-specific empirical performances but not on the information shared or missed between the models.
        \end{itemize}
    \end{frame}





==> philippe_pres/2_Deficiency.tex <==

\section{How to get rid of the downstream tasks ?}

    \begin{frame}{Relationship between embedders}
        Our objective is to compare two embedding models, $P_{U|X}$ and $P_{Z|X}$, without the need for downstream tasks.
        To do so, we want to estimate how much information on $U$ is accessible from $Z$ and vice-versa.

        \textbf{More precisely, we want to estimate how well we can simulate one embedder from the other.}
    \end{frame}

    \begin{frame}{Embedder as communication channels}
        \begin{figure}
            \centering
            \includegraphics[width=\linewidth]{Fig-NeurIPS2024}
            \caption{Communicating a concept $y\in \mathsf{Y} $ over two embedding models with prediction $\rho_Z(Z)$.}
            \label{fig:fig_channels}
        \end{figure}
    \end{frame}

    \begin{frame}{Definition of Sufficiency}
        \begin{tcolorbox}[colback=black!5!white,
                  colframe=black!75!white,
                  title=Sufficiency,
                 ]
            \begin{defn}[$U \succcurlyeq_S Z$]
                \label{def-moreinfo}
                Let $P_{U|X}$ and $P_{Z|X}$ be two Markov kernels (embedding models).

                The embedding model $P_{U|X}$ is said to be \textbf{"sufficient"} for the embedding model $P_{Z|X}$ if and only if there exists another Markov kernel $M \in \mathcal{T}(\mathsf{Z}|\mathsf{U})$  such that $\| M\!\circ\!P_{U|X} - P_{Z|X} \|_{\text{TV}}=0$.
            \end{defn}
            \tcblower

            \textit{\textbf{In other words, $U \succcurlyeq_S Z$ means that $U$ can simulate $Z$ perfectly.}}
        \end{tcolorbox}
    \end{frame}


    \begin{frame}{Sufficiency}
        \begin{tcolorbox}[colback=teal!5!white,
                  colframe=teal!75!white,
                  title=Comparison of embedding models through Bayes risks,
                 ]
            \begin{prop}\label{prop-bayes}
                Given two embedding models $P_{U|X}\in \mathcal{K}(\mathsf{U}|\mathsf{X})$ and $P_{Z|X}\in \mathcal{K}(\mathsf{Z}|\mathsf{X})$,  the following statements are equivalent:
                \begin{enumerate}
                    \item[(i)] $U \succcurlyeq_S Z$.
                    \item[(ii)] For all probability measures $P_{YX}$ on finite alphabets $\mathsf{Y}\times \mathsf{X}$, the expected Bayes risks satisfy
                    \[
                        \inf_{\rho_U:\mathsf{U}\rightarrow \mathcal{P}(\mathsf{Y})}  \Pr\big(\rho_Y(U) \neq Y \big) \leq   \inf_{\rho_Z:\mathsf{Z}\rightarrow \mathcal{P}(\mathsf{Y})} \Pr\big(\rho_Z(Z) \neq Y\big).
                    \]
                \end{enumerate}
            \end{prop}
        \end{tcolorbox}
    \end{frame}

    \begin{frame}{Sufficiency}
        \begin{tcolorbox}[colback=teal!5!white,
                  colframe=teal!75!white,
                  title=Comparison of embedding models through Bayes risks,
                 ]
            \begin{prop}\label{prop-bayes}
                Given two embedding models $P_{U|X}\in \mathcal{K}(\mathsf{U}|\mathsf{X})$ and $P_{Z|X}\in \mathcal{K}(\mathsf{Z}|\mathsf{X})$,  the following statements are equivalent:
                \begin{enumerate}
                    \item[(i)] $U \succcurlyeq_S Z$. \textbf{\textcolor{red}{U perfectly simulates Z}}
                    \item[(ii)] For all probability measures $P_{YX}$ on finite alphabets $\mathsf{Y}\times \mathsf{X}$, the expected Bayes risks satisfy
                    \[
                        \inf_{\rho_U:\mathsf{U}\rightarrow \mathcal{P}(\mathsf{Y})}  \Pr\big(\rho_Y(U) \neq Y \big) \leq   \inf_{\rho_Z:\mathsf{Z}\rightarrow \mathcal{P}(\mathsf{Y})} \Pr\big(\rho_Z(Z) \neq Y\big).
                    \]
                    \textbf{\textcolor{red}{U is better than Z on any task.}}
                \end{enumerate}

            \end{prop}
        \end{tcolorbox}
        \end{frame}

    \begin{frame}{Non-comparability}
        \begin{itemize}
            \item Equivalence: $U \succcurlyeq_S Z$ and $Z  \succcurlyeq_S U$ denoted $U \approx Z$. U and Z can simulate each other.
            \item Comparability: $U \succcurlyeq_S Z$ but $Z  \not\succcurlyeq_S U$ only Z can be simulated from U.
            \item Non-comparability: $U \not\succcurlyeq_S Z$ and $Z  \not\succcurlyeq_S U$, neither U nor Z can simulate each other.
        \end{itemize}

        \textbf{In general, two embedders are non-comparable, and no embedder can perfectly simulate another.}
    \end{frame}

    \begin{frame}[standout]{Relaxing sufficiency}
        The sufficiency is too strong to be useful in practice.
        We need to relax it to make it more tractable.
    \end{frame}

    \begin{frame}{Relaxing sufficiency}
        \begin{tcolorbox}[colback=black!5!white,
                  colframe=black!75!white,
                  title=Deficiency,
                 ]
            \begin{defn}
                \label{def:deficiency}
                The deficiency $ \delta(P_{U|X} \rightarrow P_{Z|X} ) $ of $P_{Z|X}$ relative to $P_{U|X}$ is defined as~\cite{le1964sufficiency}
                \[
                    \delta(P_{U|X} \rightarrow P_{Z|X} ) \triangleq  \inf_{M\in\mathcal{K}(\mathsf{Z}|\mathsf{U})}  \| M\!\circ\!P_{U|X} - P_{Z|X} \|_{\text{TV}},
                \]
                \end{defn}
            \tcblower
            \textbf{$ \delta$ measures error between the simulated and true embedders.}
        \end{tcolorbox}
    \end{frame}


    \begin{frame}{Relaxing sufficiency}
        \begin{tcolorbox}[colback=teal!5!white,
                  colframe=teal!75!white,
                  title=Comparison of embedding models through Bayes risks,
                 ]
            \begin{coro}\label{prop-bayes-ext}
            Given two embedding models $P_{U|X}$ and $P_{Z|X}$, the following statements are equivalent:
            \begin{enumerate}
                \item[(i)] The deficiency $ \delta(P_{U|X} \rightarrow P_{Z|X} ) \leq \epsilon $.
                \item[(ii)] For any probability distribution $P_{YX}$,
                \[
                    \mathcal{R}_U (Y) \leq  \mathcal{R}_Z (Y)+ \epsilon | \mathsf{X}|  .
                \]
            \end{enumerate}
            \end{coro}
            \tcblower
            \textbf{The performance of an embedder U compared to Z is bounded by the quality of its reconstruction of Z.}
        \end{tcolorbox}
    \end{frame}

    \begin{frame}{Deficiency and Bayesian risk}
         \[    |    \mathcal{R}_U (Y) -  \mathcal{R}_Z (Y) | \leq   | \mathsf{X}|\max\big\{ \delta(P_{U|X} \rightarrow P_{Z|X} ), \delta(P_{Z|X} \rightarrow P_{U|X} ) \big\} \]
         for all distributions $P_{YX}$. If both deficiencies are small, the resulting expected Bayes risks of the embedding models $U$ and $Z$ will be close to each other for any target task $Y$.
    \end{frame}

    \begin{frame}[standout]
        All this to say that if we can simulate an embedder from another, then the Bayes risks of the two embedders are close.
    \end{frame}

    \begin{frame}{Can we estimate the deficiency ?}

        Due to the difficulty of estimating the TV distance between two distributions, exactly estimating the deficiency is impossible.

        \textbf{As a result, we cannot directly estimate the deficiency.}
    \end{frame}


==> philippe_pres/3_is.tex <==



\section{Information sufficiency}


    \begin{frame}{Proxy of the deficiency}
        \begin{tcolorbox}[colback=black!5!white,
                  colframe=black!75!white,
                  title=Information sufficiency,
                 ]
            \begin{defn}
                The information sufficiency $ \mathcal{I}_{S}(U\rightarrow Z) $, relative to parametric classes of distributions   $\Frond_\Theta(\mathsf{Z})$ and  $\mathcal{K}_\Theta(\mathsf{Z} |\mathsf{U} )$ (multivariate Gaussian mixtures~\cite{pichler2022differential}) is defined:
                \begin{align*}
                    &\mathcal{I}_{S}(U \rightarrow Z )  \triangleq \\
                    &\underbrace{\inf_{f\in \Frond_\Theta(\mathsf{Z})} \mathbb{E}\left[ - \log f(Z) \right]}_{\text{Uncertainty of } Z} - \underbrace{\mathbb{E}\left[ \inf_{M \in \mathcal{K}_\Theta(\mathsf{Z} |\mathsf{U} ) } \mathbb{E}\left[ - \log M(Z|U) | U \right]  \right ]}_{\text{Uncertainty when simulating } Z \text{ from } U \text{ with } M}.
                \end{align*} 
            \end{defn}
        \end{tcolorbox}
    \end{frame}

    \begin{frame}{Proxy of the deficiency}
        \begin{tcolorbox}[colback=black!5!white,
                  colframe=black!75!white,
                  title=Information sufficiency,
                 ]
            \begin{defn}
                The information sufficiency $ \mathcal{I}_{S}(U\rightarrow Z) $, relative to parametric classes of distributions   $\Frond_\Theta(\mathsf{Z})$ and  $\mathcal{K}_\Theta(\mathsf{Z} |\mathsf{U} )$ (multivariate Gaussian mixtures~\cite{pichler2022differential}) is defined:
                \begin{align*}
                    &\mathcal{I}_{S}(U \rightarrow Z )  \triangleq
                    h_{\Frond_\Theta(\mathsf{Z})}(Z) - h_{\mathcal{K}_\Theta(\mathsf{Z} |\mathsf{U} ) }(Z|U).
                \end{align*}
            \end{defn}
            \tcblower
            \textbf{The information sufficiency measures how much simulating Z from U reduces the uncertainty of Z.}
        \end{tcolorbox}
    \end{frame}

    \begin{frame}{Approach}
        Our approach is the following:
        \begin{enumerate}
            \item \textbf{Encode} the data with a pool of embedders.
            \item \textbf{Estimate} the information sufficiency between the embedders.
            \item \textbf{Construct} the directed graph of the information sufficiency between models.
            \item \textbf{Compute} the ability of each embedder to simulate the others (median value).
        \end{enumerate}
    \end{frame}

    \begin{frame}{What do we do with that ?}
        \begin{columns}
            \begin{column}{0.55\linewidth}
                \begin{itemize}
                    \item \textbf{Edge}: Information sufficiency between two nodes.
                    \item \textbf{Node center}: Median information sufficiency of a node to simulate the others.
                    \item \textbf{Node edge}: Median information sufficiency of a node to be simulated by the others.
                \end{itemize}
            \end{column}
            \begin{column}{0.45\linewidth}
                \begin{figure}
                    \centering
                    \includegraphics[width=\linewidth]{fig/nlp/mteb_ds_mis_graph_community_IX_1toX_2_d_2.pdf}
                    \caption{Graph of the information sufficiency between embedders models in NLP.}
                    \label{fig:graph}
                \end{figure}
            \end{column}
        \end{columns}
    \end{frame}



==> philippe_pres/4_results.tex <==



\section{Experimental results}


    \begin{frame}{Models considered}

        \begin{table}[H]
            \centering
            \resizebox{\textwidth}{!}{
                \begin{tabular}{c| c | c |  c | c c c}
                    \toprule
                    Model name & \small SMILES & \small 2D-GNN &  \small 3D-GNN & Architecture & Out size & Dataset (size)\\
                    \midrule
                    Not-trained & & \checkmark & & \small GIN  &  300 &  - \\
                    \midrule
                    AttributeMask\cite{sun2022does} &  & \checkmark & & \small GIN  & 300 & GEOM~\cite{axelrod2022geom} \small (50k)\\
                    ContextPred\cite{sun2022does} &  & \checkmark & & \small GIN  & 300 & GEOM~\cite{axelrod2022geom} \small (50k)\\
                    GPT-GNN\cite{gptgnn} &  &  \checkmark & & \small GIN  & 300 & GEOM~\cite{axelrod2022geom} \small (50k)\\
                    InfoGraph\cite{sun2019infograph} & & \checkmark & & \small GIN  & 300 & GEOM~\cite{axelrod2022geom} \small (50k)\\
                    GraphCL\cite{You2020GraphCL} & & \checkmark & & \small GIN  & 300 & GEOM~\cite{axelrod2022geom} \small (50k)\\
                    GROVER\cite{rong2020self} & & \checkmark & & \small GIN  & 300 & GEOM~\cite{axelrod2022geom} \small (50k)\\
                    GraphLog\cite{xu2021selfsupervised} & & \checkmark & & \small GIN  & 300 & GEOM~\cite{axelrod2022geom} \small (50k)\\
                    GraphMVP\cite{liu2022pretraining}\footnotemark[1] & & \checkmark & & \small GIN  & 300 & GEOM~\cite{axelrod2022geom} \small (50k)\\
                    3D-infomax\cite{stark2021_3dinfomax}\footnotemark[1] & & \checkmark & & \small PNA & 800 & QMugs~\cite{isert2021qmugs} \small (620k)\\
                    MolR\cite{wang2022chemicalreactionaware} & & \checkmark & & \small GCN, GAT, TAG & 1024 & USPTO\cite{wang2022chemicalreactionaware} \small (~1.5M)\\
                    MoleOOD\cite{yang2022learning} & & \checkmark & & \small GIN , SAGE, GCN & 256 & BACE~\cite{hu2020ogb} \small (400k)\\
                    \midrule
                    ChemBERT \small MLM\cite{ahmad2022chemberta2} & \checkmark &  & & \small RoBERTa & 600 & PubChem~\cite{pubchem} \small (5M, 10M, 77M)\\
                    ChemBERT \small MTR\cite{ahmad2022chemberta2}  & \checkmark &  & & \small RoBERTa & 384 & PubChem~\cite{pubchem} \small (5M, 10M, 77M)\\
                    MolBert\cite{fabian2020molecular} & \checkmark &  & & \small BERT & 256 & GuacaMol~\cite{Brown_2019} \small (1.6M)\\
                    ChemGPT\cite{frey_neural_2023} & \checkmark &  & & \small GPT & 128, 256, 2048 &  PubChem~\cite{pubchem} \small (10M)\\
                    \midrule
                    3D-denosing\cite{zaidi2023pretraining} & & & \checkmark & TorchMD-net & 256 & PCQM4Mv2\cite{hu2021ogblsc} \small (3.7M)\\
                    3D-fractional\cite{pmlr-v202-feng23c} & & & \checkmark & TorchMD-net & 256 & PCQM4Mv2\cite{hu2021ogblsc} \small (3.7M)\\
                    \bottomrule
                \end{tabular}
            }
            \vspace{0.2cm}
            \caption{Molecular models compared in our study}
            \label{tab:molmodels}
        \end{table}
    \end{frame}

    \begin{frame}{Model relationship graph}
        \begin{columns}
            \begin{column}{0.4\linewidth}
                \begin{itemize}
                    \item Sequence-based models inspired from NLP are clustered together.
                    \item Various 2D models exhibit low information sufficiency, lower than the "Not-trained" baseline.
                    \item 3D models seem to be hardly simulated by other models.
                \end{itemize}
            \end{column}
            \begin{column}{0.5\linewidth}
                \begin{figure}[htbp]
                    \centering
                    \includegraphics[width=\linewidth]{fig/molecule/MI_graph_0.7}
                    \caption{Graph of the information sufficiency between the embedders.}
                    \label{fig:migraph}
                \end{figure}
            \end{column}
        \end{columns}
    \end{frame}

    \begin{frame}{Information sufficiency estimation}
        \begin{figure}
            \centering
             \begin{subfigure}{0.4\linewidth}
                 \centering
                \includegraphics[width=\linewidth]{fig/molecule/barplot_MI-3D}
                \caption{Information sufficiency of embedders in both directions.}
                \label{fig:barlot}
            \end{subfigure}
            \begin{subfigure}{0.5\linewidth}
                \centering
                \includegraphics[width=\linewidth]{fig/molecule/MI_graph_0.7}
                \caption{Graph of the information sufficiency between the embedders.}
                \label{fig:graph2}
            \end{subfigure}
        \end{figure}
    \end{frame}


    \begin{frame}{Information sufficiency estimation}
        \begin{figure}
            \centering
            \includegraphics[width=0.5\linewidth]{fig/molecule/denoising_3D_MI}
            \caption{Information sufficiency of embedders simulating 3D models, and being simulated by 3D models.}
            \label{fig:3dbarlot}
        \end{figure}
    \end{frame}


    \begin{frame}[standout]{Comparison to downstream performances}
        We now want to compare the average information sufficiency of the models, and their performance on downstream ADMET tasks.
    \end{frame}

    \begin{frame}
        \begin{table}
            \label{tab:molecul_tasks}
            \centering
            \resizebox{0.45\linewidth}{!}{
            \begin{tabular}{c c c | c c | c}
                \toprule
                Category & Model & Task & cls & reg & Avg. metric\\
                &name&size & & & in the grid\\
                \midrule
                \multirow{8}{*}{Absorption}
                & P-glycoprotein Inhibition & 1212 & \checkmark& & \textcolor{aur}{$0.88 \pm 0.03$} \\
                & AqSolDB & 9982 & & \checkmark & \textcolor{r2}{$0.52 \pm 0.09$} \\
                & Lipophilicity & 4200 & & \checkmark & \textcolor{r2}{$0.29 \pm 0.07$} \\
                 & Caco-2 Permeability & 906 & & \checkmark & \textcolor{r2}{$0.32 \pm 0.08$} \\
                & Human Intestinal Absorption & 578 & \checkmark &&  \textcolor{aur}{$0.67 \pm 0.02$} \\
                & FreeSolv & 642 & & \checkmark & \textcolor{r2}{$0.36 \pm 0.12$} \\
                & PAMPA Permeability & 2035 & \checkmark & & \textcolor{aur}{$0.67 \pm 0.02$} \\
                & Oral Bioavailability & 640 & \checkmark & & \textcolor{aur}{$0.68 \pm 0.02$} \\


                \midrule

                \multirow{3}{*}{Distribution}
                & Plasma-Protein BDR & 1614 &  & \checkmark & \textcolor{r2}{$0.18 \pm 0.04$} \\
                & Blood-Brain barrier & 1975 & \checkmark & & \textcolor{aur}{$0.32 \pm 0.08$} \\
                & VDss & 1130 & & \checkmark & \textcolor{r2}{$0.16 \pm 0.05$} \\

                \midrule

                \multirow{8}{*}{Metabolism}
                & CYPP450 3A4 Inhib. & 12328 & \checkmark & & \textcolor{aur}{$0.80 \pm 0.04$} \\
                & CYPP450 1A2 Inhib. & 12579 & \checkmark & & \textcolor{aur}{$0.87 \pm 0.03$} \\
                & CYPP450 2C19 Inhib. & 12665 & \checkmark & & \textcolor{aur}{$0.82 \pm 0.03$} \\
                & CYPP450 2C9 Inhib. & 12092 & \checkmark & & \textcolor{aur}{$0.83 \pm 0.03$} \\
                & CYPP450 2D6 Inhib. & 13130 & \checkmark & & \textcolor{aur}{$0.78 \pm 0.04$} \\
                & CYPP450 2D6 Substrate & 664 & \checkmark & & \textcolor{aur}{$0.75 \pm 0.03$} \\
                & CYPP450 3A4 Substrate & 667 & \checkmark & & \textcolor{aur}{$0.63 \pm 0.02$} \\
                & CYPP450 2C9 Substrate & 666 & \checkmark & & \textcolor{aur}{$0.65 \pm 0.02$} \\

                \midrule

                \multirow{3}{*}{Excretion}
                & Clearance hepatocyte & 1020 & & \checkmark &\textcolor{r2}{$0.11 \pm 0.03$} \\
                & Half Life & 667 & & \checkmark & \textcolor{r2}{$-0.06 \pm 0.11$} \\
                & Clearance microsome & 1102 & & \checkmark & \textcolor{r2}{$0.08 \pm 0.03$} \\

                \midrule

                \multirow{9}{*}{Toxicity}
                        & Tox21 & 7831 & \checkmark & & \textcolor{aur}{$0.75 \pm 0.03$} \\
                & \multirow{2}{*}{hERG} & 13445 & \checkmark & & \textcolor{aur}{$0.76 \pm 0.04$} \\
                &                        & 648 & \checkmark & & \textcolor{aur}{$0.75 \pm 0.03$} \\
                & Acute Toxicity LD50 & 7385 & & \checkmark & \textcolor{r2}{$0.16 \pm 0.04$} \\
                & Ames Mutagenicity & 7255 & \checkmark & &\textcolor{aur}{$0.79 \pm 0.03$} \\
                & ClinTox & 1484 & \checkmark & & \textcolor{aur}{$0.71 \pm 0.03$} \\
                & Carcinogens & 278 & \checkmark & & \textcolor{aur}{$0.76 \pm 0.08$} \\
                & Drug Induced Liver Injury & 475 & \checkmark & & \textcolor{aur}{$0.83 \pm 0.03$} \\
                & Skin Reaction & 404 & \checkmark & & \textcolor{aur}{$0.64 \pm 0.03$} \\

                \bottomrule

            \end{tabular}}
            \vspace{0.5cm}
            \caption{
                ADMET tasks extracted from the Therapeutic Data Commons platform~\cite{Huang2021tdc} considered in our experiments.
            }
            \label{tab:admet}
        \end{table}
    \end{frame}

    \begin{frame}
        \begin{figure}[htbp]
            \centering
            \begin{subtable}{.4\linewidth}
                \centering
                \resizebox{\linewidth}{!}{\input{tables/nlp/mteb_ds_overall_correlation_table_IX_1toX_2_d_2}}
                \caption{NLP}
            \end{subtable}\hspace{1.5cm}%
            \begin{subtable}{.4\linewidth}
                \centering
                \resizebox{\linewidth}{!}{\input{tables/mol/mol_glob_ranking}}
                \caption{Molecular Modelling}
            \end{subtable}
            \begin{subfigure}{0.45\textwidth}
                \centering
                \includegraphics[width=\linewidth]{fig/nlp/mteb_ds_average_scatterplot_mtebs_IX_1toX_2_d_2}
                \caption{NLP}
            \end{subfigure}\hspace{1cm}%
            \begin{subfigure}{0.45\textwidth}
                \centering
                \includegraphics[width=\linewidth]{fig/molecule/meanrank_task_size_allfig_scaff}
                \caption{Molecular Modelling}
            \end{subfigure}
            \caption{
            Global results
            }
            \label{fig:overall corr}
        \end{figure}
    \end{frame}


    \begin{frame}{Downstream tasks}
        \begin{columns}
            \begin{column}{0.55\linewidth}
                \begin{itemize}
                    \item Sequence-based models inspired from NLP exhibit poor performances (except GPT-1.2B).
                    \item \textbf{No model classified less informative than the "Not-trained" baseline outperforms it on the downstream tasks.}
                \end{itemize}
            \end{column}
            \begin{column}{0.4\linewidth}
                \begin{figure}
                    \centering
                    \includegraphics[width=\linewidth]{fig/molecule/mearnak_detailed_global_scaff}
                    \caption{Comparison of the information sufficency's rank to the rank of the models on the downstream tasks}
                    \label{fig:size}
                \end{figure}
            \end{column}
        \end{columns}
    \end{frame}




    \begin{frame}{DTI tasks}
        \begin{wrapfigure}{r}{0.6\linewidth}
            \centering
            \includegraphics[width=\linewidth]{fig/molecule/meanrank_DTI_all}
            \caption{Information sufficiency and DTI clustering task}
        \end{wrapfigure}
        We also consider the performance of the models on the DTI tasks.
        In this scenario, we are given an activity value (pXC50) for a molecule and a target.
        We considered a total of 1496 tasks.
    \end{frame}

    \begin{frame}{Size of the downstream tasks}
        \begin{figure}
            \centering
            \includegraphics[width=0.95\textwidth]{fig/molecule/correlation_task_size_scaff}
            \caption{Impact of the task size on the {\sys} score's ranking's correlation with the downstream tasks performances in molecular modeling in terms of Pearson correlation $\varrho_p$, Spearman correlation $\varrho_s$ and Kendall-Tau $\tau$ coefficient.
            }
        \end{figure}
        \textbf{When the amount of data is limited in a downstream task, the information sufficiency is not as predictive of the model's performances.}

    \end{frame}

    \begin{frame}{Number of models}
        \begin{figure}[H]
            \centering
            \includegraphics[width=0.6\linewidth]{fig/molecule/corr_kendall}
            \caption{
                Evolution of the correlation between the information sufficiency and the downstream tasks performances in molecular modeling in terms of Kendall-Tau $\tau$ coefficient.
            }
            \label{fig:models}
        \end{figure}
        \textbf{When the number of models $N$ increase, the correlation between the information sufficiency and the downstream tasks performances increases.}
    \end{frame}


==> poster/table/mint.tex <==
\begin{tabular}{r|cccccc|c}
{} & {Absorption} & {Distribution} & {Metabolism} & {Excretion} & {Tox} & {HTS} & {Avg} \\
\midrule
InfoGraph & 13.50 & 13.27 & 13.32 & 11.40 & 11.98 & 9.40 & 12.14 \\
ChemBertMLM-10M & 10.65 & 11.00 & 10.70 & 13.80 & 11.11 & 14.60 & 11.98 \\
FRAD QM9${}^{(t)}$ & 10.57 & 11.13 & 10.38 & 8.33 & 10.04 & 7.80 & 9.71 \\
ChemGPT-1.2B & 9.55 & 11.73 & 11.75 & 10.73 & 10.86 & 11.20 & 10.97 \\
GROVER & 10.43 & 8.33 & 11.25 & 8.53 & 10.38 & 11.00 & 9.99 \\
GraphCL${}^{(t)}$ & 10.89 & 8.53 & 9.45 & 10.13 & 8.70 & 9.80 & 9.58 \\
GraphLog${}^{(t)}$ & 11.05 & 7.80 & 9.07 & 10.53 & 8.93 & 14.00 & 10.23 \\
GraphMVP${}^{(t)}$ & 7.20 & 6.20 & 7.85 & 9.80 & 7.49 & 8.80 & 7.89 \\
MolR gat & 6.95 & 7.60 & 8.30 & 8.53 & 6.49 & \underline{3.40} & 6.88 \\
ThreeDInfomax${}^{(t)}$ & \underline{4.17} & \underline{6.00} & 7.58 & 7.13 & 6.16 & 10.40 & 6.91 \\
ChemBertMTR-77M${}^{(t)}$ & \textbf{\underline{3.50}} & \textbf{\underline{4.27}} & 5.75 & 5.00 & 6.03 & 4.20 & \underline{4.79} \\
\midrule
L2 & 8.07 & 6.40 & 5.55 & 6.33 & 7.55 & \textbf{3.00} & 6.15 \\
\midrule
Cosine & 5.51 & 6.13 & \underline{3.60} & \underline{4.33} & \textbf{4.97} & 6.20 & 5.13 \\
\midrule
student-250k & \textbf{3.55} & 6.20 & \textbf{\underline{2.70}} & \textbf{\underline{2.40}} & \underline{4.99} & 3.80 & \textbf{3.94} \\
student-2M & 4.40 & \textbf{5.40} & \textbf{2.75} & \textbf{3.00} & \textbf{\underline{4.34}} & \textbf{\underline{2.40}} & \textbf{\underline{3.72}} \\
\end{tabular}

